On The (In)Effectiveness of Static Logic Bomb Detector for Android Apps

Android is present in more than 85% of mobile devices, making it a prime target for malware. Malicious code is becoming increasingly sophisticated and relies on logic bombs to hide itself from dynamic analysis. In this paper, we perform a large scale study of TSOPEN, our open-source implementation of the state-of-the-art static logic bomb scanner TRIGGERSCOPE, on more than 500k Android applications. Results indicate that the approach scales. Moreover, we investigate the discrepancies and show that the approach can reach a very low false-positive rate, 0.3%, but at a particular cost, e.g., removing 90% of sensitive methods. Therefore, it might not be realistic to rely on such an approach to automatically detect all logic bombs in large datasets. However, it could be used to speed up the location of malicious code, for instance, while reverse engineering applications. We also present TRIGDB a database of 68 Android applications containing trigger-based behavior as a ground-truth to the research community.

==> appendices/overview.tex <==
\begin{figure*}[h]
\centering
\input{tikz/overview_tsopen.tikz}
\caption{Overview of TSOpen. First, the application APK is processed by \textsc{Flowdroid} to model the application. Then, every step of the analysis is applied to the ICFG until the final decision of suspiciousness of the application is taken by our tool.}
\end{figure*}



==> sections/proof.tex <==
\newtheorem*{theorem}{Theorem}
\theoremstyle{definition}
\newtheorem*{definition}{Definition}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{notations}{Notations}

\textit{\textbf{RQ1: Is it possible to automatically detect any kind of logic bomb ?}}

\begin{definition}
A logic bomb is a mechanism that modifies the control flow of a program under specific circumstances in order to trigger malicious behavior surreptitiously.
It can be defined as a pair: $(C, MC)$ where $C$ is the condition under which the malicious code is executed, i.e., the control flow is modified, and $MC$ is the malicious behavior.

In most computer languages, it can be seen as a conditional statement, i.e., an "if-then-else" statement that would trigger malicious behavior under specific circumstances.
\end{definition}

\begin{remark}
Since an algorithm can mathematically be represented by a Turing Machine~\cite{turing1937computable}, in this proof, we abstract computer programs as Turing Machines.
\end{remark}

\begin{notations}
$TM$ refers to a Turing Machine.
$\langle TM \rangle$ is used for the description of a $TM$.

\end{notations}

The problem of logic bomb detection can be stated as follow:
\[ LB \coloneqq \lbrace P \: |\: P \text{ is a } TM \text{ and } \langle P \rangle \text{ contains a logic bomb} \rbrace \]

\begin{theorem}[Undecidability of logic bomb detection]
No algorithm can decide, in a finite time, whether or not a program contains a logic bomb.
In other words, no $TM$ exists to determine, in a finite time, whether or not a sequence $S$ of a $TM$ description is a logic bomb.
\end{theorem}

\begin{proof}
We prove this assertion by contradiction.
We suppose $LB$ decidable, i.e., there is a $TM$ $D$ such as:
\[
  D (\langle P \rangle) = 
\begin{cases}
ACCEPT & \text{if } \langle P \rangle \text{ contains a logic bomb} \\
  REJECT & \text{otherwise}
\end{cases}
\]
Note that $D$ always terminates.

We consider a new $TM$ $P'$ whose description $\langle P' \rangle$ contains a logic bomb $(c,v)$ with $c$ any condition and $v$ a self-replicating virus.
We suppose the rest of $\langle P' \rangle$ free from malicious behavior.
In other words : 
\[ D (\langle P' \rangle) = ACCEPT \]

\begin{remark}
A virus is not necessarily malicious, but in this case, we consider $v$ malicious as it is part of a logic bomb.
$P'$ can thus be represented by the intersection of the two hatched parts in Figure~\ref{sets}. 

\end{remark}

\begin{figure}
\centering
\input{tikz/sets.tikz}
\caption{Malicious programs, viruses and programs with logic bomb representation.}
\label{sets}
\end{figure}

We can construct a new $TM$ $V$ which decides whether or not $\langle P' \rangle$ contains a viral sequence, here $v$, i.e., $P'$ is a virus, such as:

$V =$ "On input $\langle P' \rangle$
\begin{enumerate}[leftmargin=1.5cm]
\item Run $D$ on input $\langle P' \rangle$
\item Agree with D answer"
\end{enumerate}

Hence:
\[
  V (\langle P' \rangle) = 
\begin{cases}
ACCEPT & \text{if } D \; ACCEPTS \; \langle P' \rangle \\
REJECT & \text{if } D \; REJECTS \; \langle P' \rangle
\end{cases}
\]
Thus we have a Turing Machine deciding whether a given sequence in a given Turing Machine is a viral sequence ($\Rightarrow \! \Leftarrow$).
This is a contradiction since we know, from Cohen's previous work~\cite{cohen1986computer}, that $V$ cannot exist due to its undecidability (Virus set in Figure~\ref{sets}), hence $D$ cannot exist.

Therefore, we have demonstrated that no Turing Machine, i.e., no algorithm, can exist to resolve the logic bomb detection problem in a finite time.
\end{proof}

\fbox{\begin{minipage}{0.9\columnwidth}
We have demonstrated that the problem of detecting logic bombs is undecidable. Therefore, it is impossible to automatically detect all logic bombs in a finite amount of time.
That is why, in practice, we have to approximate by using heuristics in order to improve the detection of such mechanisms.
\end{minipage}}

==> sections/rqfpr_apppkgfilter.tex <==


The package filter in this experiment aims at not taking into account any potential logic bomb detected by \tso{} if the package in which the method containing the trigger is not the same as the package of the Android application considered.
%
The number of triggers still stays high, falling from 5391 to 2004.
The number of applications containing at least one potential logic bomb drops from 1701 to 617.
Therefore, the potential rate of false-positive falls from 23.3\% to 8.4\%.
\ab{Unfortunately, the analysis does not take into account all the code outside of the package.
In some applications this accounts for more than XX\% of the code.}

\myshortconclusion{
Using a package filter can impact the false positive rate of at least one order of magnitude.
}

